A Bandit Approach to Online Pricing for Heterogeneous Edge Resource Allocation

Edge Computing (EC) offers a superior user experience by positioning cloud resources in close proximity to end users. The challenge of allocating edge resources efficiently while maximizing profit for the EC platform remains a sophisticated problem, especially with the added complexity of the online arrival of resource requests. To address this challenge, we propose to cast the problem as a multi-armed bandit problem and develop two novel online pricing mechanisms, the Kullback-Leibler Upper Confidence Bound (KL-UCB) algorithm and the Min-Max Optimal algorithm, for heterogeneous edge resource allocation. These mechanisms operate in real-time and do not require prior knowledge of demand distribution, which can be difficult to obtain in practice. The proposed posted pricing schemes allow users to select and pay for their preferred resources, with the platform dynamically adjusting resource prices based on observed historical data. Numerical results show the advantages of the proposed mechanisms compared to several benchmark schemes derived from traditional bandit algorithms, including the Epsilon-Greedy, basic UCB, and Thompson Sampling algorithms.

==> CapRef.tex <==
%%%%%%%%%%%%%%%%% Survey Dynamic pricing %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{kumar2018survey,
  title={A survey on spot pricing in cloud computing},
  author={Kumar, Dinesh and Baranwal, Gaurav and Raza, Zahid and Vidyarthi, Deo Prakash},
  journal={Journal of Network and Systems Management},
  volume={26},
  number={4},
  pages={809--856},
  year={2018},
  publisher={Springer}
}


%%%%%%%%% Survey in Edge Computing %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@techreport{carpenter02,
  title={Middleboxes: Taxonomy and issues},
  author={Carpenter, Brian and Brim, Scott},
  year={2002},
  institution={RFC 3234, February}
}

@ARTICLE{mchi16,
  author={Chiang, Mung and Zhang, Tao},
  journal={IEEE Internet  Things J.}, 
  title={Fog and IoT: {A}n Overview of Research Opportunities}, 
  year={2016},
  volume={3},
  number={6},
  pages={854-864},
  doi={10.1109/JIOT.2016.2584538}}


@ARTICLE{wshi16,
  author={Shi, Weisong and Cao, Jie and Zhang, Quan and Li, Youhuizi and Xu, Lanyu},
  journal={IEEE Internet  Things J.}, 
  title={Edge Computing: Vision and Challenges}, 
  year={2016},
  volume={3},
  number={5},
  pages={637-646},
  doi={10.1109/JIOT.2016.2579198}}


@article{NFV_review,
  title={Network function virtualization: Challenges and opportunities for innovations},
  author={Han, Bo and Gopalakrishnan, Vijay and Ji, Lusheng and Lee, Seungjoon},
  journal={IEEE Commun. Mag.},
  volume={53},
  number={2},
  pages={90--97},
  year={2015},
  publisher={IEEE}
}

%%%%%%%%% Pricing %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{double18,
  author={Sun, Wen and Liu, Jiajia and Yue, Yanlin and Zhang, Haibin},
  journal={IEEE Trans Ind. Informat.}, 
  title={Double {A}uction-{B}ased {R}esource {A}llocation for {M}obile {E}dge {C}omputing in {I}ndustrial {I}nternet of {T}hings}, 
  year={2018},
  volume={14},
  number={10},
  pages={4692-4701},
  doi={10.1109/TII.2018.2855746}}


@ARTICLE{Duong_TON,
  author={Nguyen, Duong Tung and Le, Long Bao and Bhargava, Vijay K.},
  journal={IEEE/ACM Trans. Netw.}, 
  title={A {M}arket-{B}ased {F}ramework for {M}ulti-{R}esource {A}llocation in {F}og {C}omputing}, 
  year={2019},
  volume={27},
  number={3},
  pages={1151-1164},
  doi={10.1109/TNET.2019.2912077}}


@ARTICLE{Duong_TCC,
  author={Nguyen, Duong Tung and Le, Long Bao and Bhargava, Vijay},
  journal={IEEE Trans. Cloud Comput.}, 
  title={Price-{B}ased {R}esource {A}llocation for {E}dge {C}omputing: {A} {M}arket {E}quilibrium {A}pproach}, 
  year={2021},
  volume={9},
  number={1},
  pages={302-317},
  doi={10.1109/TCC.2018.2844379}}


@ARTICLE{tara22,
  author={Nisha, Tarannum and Nguyen, Duong Tung and Bhargava, Vijay K.},
  journal={IEEE Internet Things J.}, 
  title={A {B}ilevel {P}rogramming {F}ramework for {J}oint {E}dge {R}esource {M}anagement and {P}ricing}, 
  year={2022},
  volume={9},
  number={18},
  pages={17280--17291},
  doi={10.1109/JIOT.2022.3152139}}


@article{jyan21,
  title={Pricing-{D}riven {S}ervice {C}aching and {T}ask {O}ffloading in {M}obile {E}dge {C}omputing},
  author={Yan, Jia and Bi, Suzhi and Duan, Lingjie and Zhang, Ying-Jun Angela},
  journal={IEEE Trans. Wireless Commun.},
  volume={20},
  number={7},
  pages={4495--4512},
  year={2021},
  publisher={IEEE}
}

  @inproceedings{auction21,
  title={Auction-{B}ased {C}ombinatorial {M}ulti-{A}rmed {B}andit {M}echanisms with {S}trategic {A}rms},
  author={Gao, Guoju and Huang, He and Xiao, Mingjun and Wu, Jie and Sun, Yu-E and Zhang, Sheng},
  booktitle={Proc. IEEE INFOCOM},
  pages={1--10},
  year={2021},
  organization={IEEE}
}

%%%%%%%%%%% Dynamic pricing in edge computing %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{chuan17,
  title={Optimal posted prices for online cloud resource allocation},
  author={Zhang, Zijun and Li, Zongpeng and Wu, Chuan},
  journal={Proc.ACM Measurement and Analysis of Comput. Syst.},
  volume={1},
  number={1},
  pages={1--26},
  year={2017},
  publisher={ACM New York, NY, USA}
}

    
 @ARTICLE{zhang17,
  author={Zhang, Xiaoxi and Huang, Zhiyi and Wu, Chuan and Li, Zongpeng and Lau, Francis C. M.},
  journal={IEEE/ACM Trans. Netw}, 
  title={Online {A}uctions in {I}aaS {C}louds: {W}elfare and {P}rofit {M}aximization {W}ith {S}erver {C}osts}, 
  year={2017},
  volume={25},
  number={2},
  pages={1034-1047}}
  
  
@ARTICLE{Yang22,
  author={Yang, Chien-Sheng and Pedarsani, Ramtin and Avestimehr, A. Salman},
  journal={IEEE/ACM Trans. Netw.}, 
  title={Edge computing in the dark: leveraging contextual-combinatorial bandit and coded computing}, 
  year={2021},
  volume={29},
  number={3},
  pages={1022--1031},
  doi={10.1109/TNET.2021.3058685}}

@article{Qu18,
  title={Posted {P}ricing for {C}hance {C}onstrained {R}obust {C}rowdsensing},
  author={Qu, Yuben and Tang, Shaojie and Dong, Chao and Li, Peng and Guo, Song and Dai, Haipeng and Wu, Fan},
  journal={IEEE Trans. Mobile Comput.},
  volume={19},
  number={1},
  pages={188--199},
  year={2018},
  publisher={IEEE}
}


@inproceedings{xuehe19,
  title={Dynamic pricing and capacity allocation of {UAV}-provided mobile services},
  author={Wang, Xuehe and Duan, Lingjie},
  booktitle={Proc. IEEE INFOCOM},
  pages={1855--1863},
  year={2019},
  organization={IEEE}
}

@inproceedings{siew21,
  title={Let’s share vms: Optimal placement and pricing across base stations in mec systems},
  author={Siew, Marie and Guo, Kun and Cai, Desmond and Li, Lingxiang and Quek, Tony QS},
  booktitle={Proc. IEEE INFOCOM},
  pages={1--10},
  year={2021},
  organization={IEEE}
}

@inproceedings{ofm19,
  title={{OFM}: {A}n {O}nline {F}isher {M}arket for {C}loud {C}omputing},
  author={Prasad, Abhinandan S and Arumaithurai, Mayutan and Koll, David and Jiang, Yuming and Fu, Xiaoming},
  booktitle={Proc. INFOCOM},
  pages={2575--2583},
  year={2019},
  organization={IEEE}
}

@article{zhu18,
  title={Truthful online auction toward maximized instance utilization in the cloud},
  author={Zhu, Yifei and Fu, Silvery D and Liu, Jiangchuan and Cui, Yong},
  journal={IEEE/ACM Trans. Netw.},
  volume={26},
  number={5},
  pages={2132--2145},
  year={2018},
  publisher={IEEE}
}

@ARTICLE{Danny20,
  author={Tan, Xiaoqi and Leon-Garcia, Alberto and Wu, Yuan and Tsang, Danny H. K.},
  journal={IEEE J. Sel. Areas Commun.}, 
  title={Online {C}ombinatorial {A}uctions for {R}esource {A}llocation {W}ith {S}upply {C}osts and {C}apacity {L}imits}, 
  year={2020},
  volume={38},
  number={4},
  pages={655--668}}

@ARTICLE{jun20,
  author={Li, Gang and Cai, Jun},
  journal={IEEE Internet Things J.}, 
  title={An {O}nline {I}ncentive {M}echanism for {C}rowdsensing {W}ith {R}andom {T}ask {A}rrivals}, 
  year={2020},
  volume={7},
  number={4},
  pages={2982--2995},
  doi={10.1109/JIOT.2020.2964657}}

@article{three21,
  title={Three-{S}tage {S}tackelberg {L}ong-term {I}ncentive {M}echanism and {M}onetization for {M}obile {C}rowdsensing: {A}n {O}nline {L}earning {A}pproach},
  author={Li, Youqi and Li, Fan and Yang, Song and Zhou, Pan and Zhu, Liehuang and Wang, Yu},
  journal={IEEE Trans. Netw. sci. Eng.},
  volume={8},
  number={2},
  pages={1385--1398},
  year={2021}}

@article{ella2022,
	author = {Nguyen, Duong Thuy Anh and Cheng, Jiaming and Trieu, Ni and Nguyen, Duong Tung},
    title = {A {F}airness-{A}ware {A}ttacker-{D}efender {M}odel for {O}ptimal {E}dge {N}etwork {O}peration and {P}rotection},
	journal={arXiv preprint arXiv:2301.06644},
	year={2022}}

 @ARTICLE{zhang21,
  author={Zhang, Xiaoxi and Huang, Zhiyi and Wu, Chuan and Li, Zongpeng and Lau, Francis C. M.},
  journal={IEEE Trans. Cloud Comput.}, 
  title={Dynamic {VM} {S}caling: {P}rovisioning and {P}ricing through an {O}nline {A}uction}, 
  year={2021},
  volume={9},
  number={1},
  pages={131--144}} 


@ARTICLE{Zhou22,
  author={Zhou, Ruiting and Wang, Ne and Huang, Yifeng and Pang, Jinlong and Chen, Hao},
  journal={IEEE Trans, Mob. Comput.}, 
  title={DPS: Dynamic Pricing and Scheduling for Distributed Machine Learning Jobs in Edge-Cloud Networks}, 
  year={2022},
  volume={},
  number={},
  pages={1--16},
  doi={10.1109/TMC.2022.3195765}}


@ARTICLE{Wang22,
  author={Wang, Xiong and Ye, Jiancheng and Lui, John C.S.},
  journal={IEEE/ACM Trans. Netw.}, 
  title={Decentralized scheduling and dynamic pricing for edge computing: a mean field game approach}, 
  year={2022},
  pages={1--14}}



%%%%%%%%%%%%%%%%%%%%%%%Bandit pricing %%%%%%%%%%%%%%%% 


@INPROCEEDINGS{Chuan18,
  author={Zhang, Xiaoxi and Wu, Chuan and Huang, Zhiyi and Li, Zongpeng},
  booktitle={Proc. IEEE INFOCOM}, 
  title={Occupation-{O}blivious {P}ricing of {C}loud {J}obs via {O}nline {L}earning}, 
  year={2018},
  pages={2456--2464}}

@INPROCEEDINGS{RL22,
  author={Lyu, Feng and Cai, Xinyao and Wu, Fan and Lu, Huali and Duan, Sijing and Ren, Ju},
  booktitle={Proc. IEEE/ACM IWQoS}, 
  title={Dynamic Pricing Scheme for Edge Computing Services: A Two-layer Reinforcement Learning Approach}, 
  year={2022},
  pages={1--10}}


@inproceedings{time22,
  title={Online {P}ricing with {L}imited {S}upply and {T}ime-{S}ensitive {V}aluations},
  author={Li, Shaoang and Zhang, Lan and Li, Xiang-Yang},
  booktitle={Proc. IEEE INFOCOM},
  pages={860--869},
  year={2022},
  organization={IEEE}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Myerson81,
  title={Optimal {A}uction {D}esign},
  author={R. B. Myerson},
  journal={Mathematics of Operations Research},
  volume={1},
  number={6},
  pages={58--73},
  year={1981},
  publisher={SIAM}
}


@INPROCEEDINGS{duong_wfiot,
  author={Nguyen, Duong Tung and Le, Long Bao and Bhargava, Vijay},
  booktitle={Proc. IEEE WF-IoT}, 
  title={Edge computing resource procurement: An online optimization approach}, 
  year={2018},
  volume={},
  number={},
  pages={807-812},
  doi={10.1109/WF-IoT.2018.8355134}}

%%%%%%%%% DATA SOURCE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@inproceedings{Hotedge,
  title={Benchmarking in the dark: On the absence of comprehensive edge datasets},
  author={Kolosov, Oleg and Yadgar, Gala and Maheshwari, Sumit and Soljanin, Emina},
  booktitle={USENIX HotEdge},
  year={2020}
}

  %%%%%%%%%%%%%%%%%%%%%%% Bandit/Online optimization %%%%%%%%%%%%%%%%%
@inproceedings{Kleinberg2008, author = {Kleinberg, Robert and Slivkins, Aleksandrs and Upfal, Eli}, title = {Multi-Armed Bandits in Metric Spaces}, year = {2008}, isbn = {9781605580470}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, url = {https://doi.org/10.1145/1374376.1374475}, doi = {10.1145/1374376.1374475}, booktitle = {Proceedings of the Fortieth Annual ACM Symposium on Theory of Computing}, pages = {681–690}, numpages = {10}, keywords = {online learning, covering dimension, metric spaces, multi-armed bandit problem}, location = {Victoria, British Columbia, Canada}, series = {STOC '08} }

@inproceedings {Sekar12,
    author = {Vyas Sekar and Norbert Egi and Sylvia Ratnasamy and Michael K. Reiter and Guangyu Shi},
    title = {Design and Implementation of a Consolidated Middlebox Architecture},
    booktitle = {Proc. USENIX NSDI},
    year = {2012},
    address = {San Jose, CA},
    pages = {323--336},
    publisher = {USENIX Association}}
 

@article{auer2002,
  title={Finite-time {A}nalysis of the {M}ulti-{A}rmed {B}andit {P}roblem},
  author={Auer, Peter and Cesa-Bianchi, Nicolo and Fischer, Paul},
  journal={Machine learning},
  volume={47},
  number={2},
  pages={235--256},
  year={2002},
  publisher={Springer}
}


@inproceedings{nips11,
 author = {Slivkins, Aleksandrs},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {J. Shawe-Taylor and R. Zemel and P. Bartlett and F. Pereira and K.Q. Weinberger},
 title = {Multi-armed bandits on implicit metric spaces},
 volume = {24},
 year = {2011}
}

%%% bandit %%%%%%%%%%%%%%%

@article{DPbandit19,
author = {Misra, Kanishka and Schwartz, Eric M. and Abernethy, Jacob},
title = {Dynamic Online Pricing with Incomplete Information Using Multi armed Bandit Experiments},
year = {2019},
issue_date = {March-April 2019},
publisher = {INFORMS},
address = {Linthicum, MD, USA},
volume = {38},
number = {2},
issn = {1526-548X},
url = {https://doi.org/10.1287/mksc.2018.1129},
doi = {10.1287/mksc.2018.1129},
journal = {Marketing Science},
month = {Mar.},
pages = {226–252},
numpages = {27},
keywords = {minimax regret, machine learning, partial identification, dynamic pricing, A/B testing, field experiments, nonparametric econometrics, online experiments, e-commerce, multiarmed bandits}
}

@article{UCB,
  title={Finite-time analysis of the multiarmed bandit problem},
  author={Auer, Peter and Cesa-Bianchi, Nicolo and Fischer, Paul},
  journal={Machine learning},
  volume={47},
  number={2},
  pages={235--256},
  year={2002},
}

@inproceedings{Epislongreedy,
  title={Classes of {M}ultiagent {Q}-learning {D}ynamics with epsilon-greedy {E}xploration},
  author={Wunder, Michael and Littman, Michael L and Babes, Monica},
  booktitle={ICML},
  year={2010}
}

@article{EXP3,
  title={The nonstochastic multiarmed bandit problem},
  author={Auer, Peter and Cesa-Bianchi, Nicolo and Freund, Yoav and Schapire, Robert E},
  journal={SIAM journal on computing},
  volume={32},
  number={1},
  pages={48--77},
  year={2002},
  publisher={SIAM}
}

@article{CappedUCB,
author = {Babaioff, Moshe and Dughmi, Shaddin and Kleinberg, Robert and Slivkins, Aleksandrs},
title = {Dynamic Pricing with Limited Supply},
address = {New York, NY, USA},
volume = {3},
number = {1},
pages = {2167--8375},
journal = {ACM Trans. Econ. Comput.},
month = {mar},
year = {2015},
pages = {26}}


@inproceedings{KLUCB,
  title={The {KL-UCB} {A}lgorithm for {B}ounded {S}tochastic {B}andits and {B}eyond},
  author={Garivier, Aur{\'e}lien and Capp{\'e}, Olivier},
  booktitle={Proc. COLT},
  pages={359--376},
  year={2011},
  organization={JMLR Workshop and Conference Proceedings}
}

@inproceedings{MOSS,
  title={Minimax {P}olicies for {A}dversarial and {S}tochastic {B}andits},
  author={Audibert, Jean-Yves and Bubeck, S{\'e}bastien},
  booktitle={Proc. COLT},
  volume={7},
  pages={1--122},
  year={2009}
}

@ARTICLE{Ghoorchian2021,
  author={Ghoorchian, Saeed and Maghsudi, Setareh},
  journal={IEEE Trans. Cogn. Commun. Netw. }, 
  title={Multi-{A}rmed {B}andit for {E}nergy-{E}fficient and {D}elay-{S}ensitive {E}dge {C}omputing in {D}ynamic {N}etworks {W}ith {U}ncertainty}, 
  year={2021},
  volume={7},
  number={1},
  pages={279-293},
  doi={10.1109/TCCN.2020.3012445}}


@inproceedings{TS,
  title={Thompson {S}ampling: {A}n {A}symptotically {O}ptimal {F}inite-{T}ime {A}nalysis},
  author={Kaufmann, Emilie and Korda, Nathaniel and Munos, R{\'e}mi},
  booktitle={Proc. ALT},
  pages={199--213},
  year={2012},
  organization={Springer}
}

@INPROCEEDINGS{Kleinberg03,
  author={Kleinberg, R. and Leighton, T.},
  booktitle={Proc. FOCS}, 
  title={The value of knowing a demand curve: bounds on regret for online posted-price auctions}, 
  year={2003},
  pages={594-605},
  doi={10.1109/SFCS.2003.1238232}}


@article{laibound,
  title={Asymptotically {E}fficient {A}daptive {A}llocation {R}ules},
  author={Lai, Tze Leung and Robbins, Herbert and others},
  journal={Advances in applied mathematics},
  volume={6},
  number={1},
  pages={4--22},
  year={1985}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% data source %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@misc{Materna,
    note  = {\url{http://gwa.ewi.tudelft.nl/datasets/gwa-t-13-materna}, 
             Access Dec 2021},
}

@misc{EC2,
    title = {Amazon {EC2} instance},
    note  = {\url{https://aws.amazon.com/ec2/instance-types/}, 
             Access Sep 2022},
}

@article{Ashwinkumar2018, 
    author = {Badanidiyuru, Ashwinkumar and Kleinberg, Robert and Slivkins, Aleksandrs}, 
    title = {Bandits with Knapsacks}, 
    year = {2018}, 
    issue_date = {June 2018}, 
    publisher = {Association for Computing Machinery}, 
    address = {New York, NY, USA}, 
    volume = {65}, 
    number = {3}
}

@inproceedings{Badanidiyuru2013BanditsWK,
  title={Bandits with Knapsacks: Dynamic procurement for crowdsourcing},
  author={Ashwinkumar Badanidiyuru and Robert D. Kleinberg and Aleksandrs Slivkins},
  year={2013}
}

@misc{wondernetwork,
    title = {Global Ping Statistics},
    note  = {\url{https://wondernetwork.com/pings}, 
             Access Dec 2021},
}


@misc{equinix,
    note  = {\url{https://www.equinix.nl/data-centers}, 
             Access Dec 2021},
}



